Social Media Identity Deception Detection: A Survey

Social media have been growing rapidly and become essential elements of many people's lives. Meanwhile, social media have also come to be a popular source for identity deception. Many social media identity deception cases have arisen over the past few years. Recent studies have been conducted to prevent and detect identity deception. This survey analyses various identity deception attacks, which can be categorized into fake profile, identity theft and identity cloning. This survey provides a detailed review of social media identity deception detection techniques. It also identifies primary research challenges and issues in the existing detection techniques. This article is expected to benefit both researchers and social media providers.

==> extra.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}[
  level 1/.style={sibling distance=40mm},
  edge from parent/.style={->,draw},
  >=latex]
% root of the the initial tree, level 1
\node[root] {Social Media Identity Deception Attacks}
% The first level, as children of the initial tree
  child {node[level 2] (c1) {Fake Profile}}
  child {node[level 2] (c2) {Identity Theft}}
  child {node[level 2] (c3) {Identity Cloning}};
% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level 2}]
\node [below of = c1, xshift=15pt] (c11) {Sybil Attack};
\node [below of = c11] (c12) {Sockpuppets};
\node [below of = c12] (c13) {Social Botnet};
\node [below of = c13] (c14) {Spammers};

\node [below of = c2, xshift=15pt] (c21) {Compromised Account};
\node [below of = c21] (c22) {Hijacked Account};

\node [below of = c3, xshift=15pt] (c31) {Single Site};
\node [below of = c31] (c32) {Cross Site};

\end{scope}

% lines from each level 1 node to every one of its "children"
\foreach \value in {1,2,3,4}
  \draw[->] (c1.190) |- (c1\value.west);

\foreach \value in {1,2}
  \draw[->] (c2.190) |- (c2\value.west);

\foreach \value in {1,2}
  \draw[->] (c3.190) |- (c3\value.west);
\end{tikzpicture}
\caption{Identity deception attacks on social media platforms \textbf{can you make fig.2 more compact?}} \label{identity_attacks}

\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
